Geometric Aspects and Testing of the Galactic Center Distance Determination from Spiral Arm Segments

We consider the problem of determining the geometric parameters of a Galactic spiral arm from its segment by including the distance to the spiral pole, i.e., the distance to the Galactic center ($R_0$). The question about the number of points belonging to one turn of a logarithmic spiral and defining this spiral as a geometric figure has been investigated numerically and analytically by assuming the direction to the spiral pole (to the Galactic center) to be known. Based on the results obtained, in an effort to test the new approach, we have constructed a simplified method of solving the problem that consists in finding the median of the values for each parameter from all possible triplets of objects in the spiral arm segment satisfying the condition for the angular distance between objects. Applying the method to the data on the spatial distribution of masers in the Perseus and Scutum arms (the catalogue by Reid et al. (2014)) has led to an estimate of $R_0 = 8.8 \pm 0.5$ kpc. The parameters of five spiral arm segments have been determined from masers of the same catalogue. We have confirmed the difference between the spiral arms in pitch angle. The pitch angles of the arms revealed by masers are shown to generally correlate with $R_0$ in the sense that an increase in $R_0$ leads to a growth in the absolute values of the pitch angles.

==> ps2pdffonts <==
#!/bin/bash
#/bin/bash -x
# ps2pdf with preserving fonts in eps files made via gnuplot
# Tit --- > Nii 1.0 

syn="Synopsis:
     $0 ps-file"

if [ $# -ne 1 ]; then
    echo $0: no or too much file names: $1
    echo $syn; exit 1
fi

ps2pdf -dPDFSETTINGS=/prepress -dAutoRotatePages=/None -dEmbedAllFonts=true \
       -dSubsetFonts=true $1

